Better May Not Be Fairer: A Study on Subgroup Discrepancy in Image Classification

In this paper, we provide 20,000 non-trivial human annotations on popular datasets as a first step to bridge gap to studying how natural semantic spurious features affect image classification, as prior works often study datasets mixing low-level features due to limitations in accessing realistic datasets. We investigate how natural background colors play a role as spurious features by annotating the test sets of CIFAR10 and CIFAR100 into subgroups based on the background color of each image. We name our datasets \textbf{CIFAR10-B} and \textbf{CIFAR100-B} and integrate them with CIFAR-Cs. We find that overall human-level accuracy does not guarantee consistent subgroup performances, and the phenomenon remains even on models pre-trained on ImageNet or after data augmentation (DA). To alleviate this issue, we propose \textbf{FlowAug}, a \emph{semantic} DA that leverages decoupled semantic representations captured by a pre-trained generative flow. Experimental results show that FlowAug achieves more consistent subgroup results than other types of DA methods on CIFAR10/100 and on CIFAR10/100-C. Additionally, it shows better generalization performance. Furthermore, we propose a generic metric, \emph{MacroStd}, for studying model robustness to spurious correlations, where we take a macro average on the weighted standard deviations across different classes. We show \textit{MacroStd} being more predictive of better performances; per our metric, FlowAug demonstrates improvements on subgroup discrepancy. Although this metric is proposed to study our curated datasets, it applies to all datasets that have subgroups or subclasses. Lastly, we also show superior out-of-distribution results on CIFAR10.1.

==> algorithm1.tex <==
% \begin{minipage}{\textwidth}
% \centering
% \begin{minipage}{0.49\textwidth}

%     % \begin{wrapfigure}{r}{0.5\textwidth}
        
%         % \begin{minipage}{0.5\textwidth}
%         % \vspace{-10pt}
%         \begin{algorithm}%[H]
%         \caption{FlowAug-Gaussian}\label{alg:gaussian}
%         \label{alg}
%             \KwInput{Flow: $\mathcal{F}$, Dataset: $X$, $L$, $\mu, \sigma, b$}
%             \For{$l = 1, ..., L$}
%             {  
%               $x\sim X$\tcp*{Sample image}
%               $z,\nu \leftarrow \mathcal{F}_{enc}(x)$ \tcp*{Encode the image}
%               $\epsilon \sim \mathcal{N}_{trunc}(\mu,\sigma^2;b) $\tcp*{Sample perturbations}
%               $z \leftarrow z + \epsilon $\tcp*{explore space} 
%               $x_{aug} \leftarrow \mathcal{F}_{dec}(z,\nu)$ \tcp*{Decode global and local back to image space}
%             }
%             \KwOutput{$X_{aug}$}
%         \end{algorithm}
%         % \end{minipage}
%     % \end{wrapfigure}
% \end{minipage}
% \begin{minipage}{0.5\textwidth}
% \begin{figure*}[t]
    %  \centering
    %  \includegraphics[width=1\textwidth]{figures/graphical.png}
    %     \captionof{figure}{\textbf{Graphical model depicting our disentanglement assumptions.}}
    %     \label{fig:graphical}
% \end{figure*}
% \end{minipage}
% \end{minipage}


\begin{algorithm}%[H]
        \caption{FlowAug-Gaussian Global $z$}\label{alg:gaussian}
        \label{alg}
            \KwInput{Flow: $\mathcal{F}$, Dataset: $X$, $L$, $\mu, \sigma, b$}
            \For{$l = 1, ..., L$}
            {  
               $x\sim X$\tcp*{Sample image}
               $z,\nu \leftarrow \mathcal{F}_{enc}(x)$ \tcp*{Encode the image}
               $\epsilon \sim \mathcal{N}_{trunc}(\mu,\sigma^2;b) $\tcp*{Sample perturbations}
               $z \leftarrow z + \epsilon $\tcp*{explore space} 
               $x_{aug} \leftarrow \mathcal{F}_{dec}(z,\nu)$ \tcp*{Decode global and local back to image space}
            }
            \KwOutput{$X_{aug}$}
\end{algorithm}
        
% \begin{figure*}[t]
%      \centering
%      \includegraphics[width=\linewidth]{figures/graphical.png}
%         \captionof{figure}{\textbf{Graphical model depicting our disentanglement assumptions.}}
%         \label{fig:graphical}
% \end{figure*}

==> algorithm2.tex <==
% \begin{wrapfigure}{r}{0.5\textwidth}
% % \vspace{.5em}
%     \begin{algorithm}%[H]
%     \caption{FlowAug-Mix $z$}\label{alg:mix}
%     \label{alg}
%         \KwInput{Flow: $\mathcal{F}$, Dataset: $X$, Threshold: $tr$, $L$, $\alpha$}
%         \For{$l = 1, ..., L$}
%         {  $x_1, x_2 \sim X$\tcp*{Sample images}
%           $z_1,\nu_1 \leftarrow \mathcal{F}_{enc}(x_1)$ \tcp*{Encode $x_1$}
%           $z_2,\nu_2 \leftarrow \mathcal{F}_{enc}(x_2)$ \tcp*{Encode $x_2$}
%           $m\sim Beta(\alpha,\alpha)$\tcp*{Sample interpolation parameter}
%           \If{$m < tr$}{
%                   $m\leftarrow1-m$ \tcp*{Avoid drastic change in $style$}
%           }
%           $z_1 \leftarrow m z_1 + (1-m) z_2$\tcp*{explore space} 
%           $x_{aug} \leftarrow \mathcal{F}_{dec}(z_1,\nu_1)$ \tcp*{Decode global and local}
%         }
%         \KwOutput{$X_{aug}$}
        
%     \end{algorithm}
% \end{wrapfigure}
% % \hfil
\begin{algorithm}%[H]
    \caption{FlowAug-Mix Gloabl $z$}\label{alg:mix}
    \label{alg}
        \KwInput{Flow: $\mathcal{F}$, Dataset: $X$, Threshold: $tr$, $L$, $\alpha$}
        \For{$l = 1, ..., L$}
        {  $x_1, x_2 \sim X$\tcp*{Sample images}
           $z_1,\nu_1 \leftarrow \mathcal{F}_{enc}(x_1)$ \tcp*{Encode $x_1$}
           $z_2,\nu_2 \leftarrow \mathcal{F}_{enc}(x_2)$ \tcp*{Encode $x_2$}
           $m\sim Beta(\alpha,\alpha)$\tcp*{Sample interpolation parameter}
           \If{$m < tr$}{
                  $m\leftarrow1-m$ \tcp*{Avoid drastic change in $style$}
           }
           $z_1 \leftarrow m z_1 + (1-m) z_2$\tcp*{explore space} 
           $x_{aug} \leftarrow \mathcal{F}_{dec}(z_1,\nu_1)$ \tcp*{Decode global and local}
        }
        \KwOutput{$X_{aug}$}
        
\end{algorithm}

==> aug_methods_fig.tex <==
\begin{figure*}[t]
     \begin{subfigure}[t]{0.24\textwidth}
         \centering \includegraphics[scale=1.3]{figures/augmentations/natural.png}
         \caption{Original}
     \end{subfigure}
     \begin{subfigure}[t]{0.24\textwidth}
         \centering \includegraphics[scale=1.3]{figures/augmentations/mixup.png}
         \caption{MixUp}
     \end{subfigure}
     \begin{subfigure}[t]{0.24\textwidth}
         \centering \includegraphics[scale=1.3]{figures/augmentations/cutout.png}
         \caption{Cutout}
     \end{subfigure}
     \begin{subfigure}[t]{0.24\textwidth}
         \centering \includegraphics[scale=1.3]{figures/augmentations/cutmix.png}
         \caption{Cutmix}
     \end{subfigure}
     
     
     \begin{subfigure}[t]{0.24\textwidth}
         \centering \includegraphics[scale=1.3]{figures/augmentations/autoaug.png}
         \caption{AutoAug (invert)}
     \end{subfigure}
     \begin{subfigure}[t]{0.24\textwidth}
         \centering \includegraphics[scale=1.3]{figures/augmentations/switch_global.png}
         \caption{Mix Global $z$}
     \end{subfigure}
     \begin{subfigure}[t]{0.24\textwidth}
         \centering \includegraphics[scale=1.3]{figures/augmentations/gaussian_glo.png}
         \caption{Gaussian Global $z$}
     \end{subfigure}
     \begin{subfigure}[t]{0.24\textwidth}
         \centering \includegraphics[scale=1.3]{figures/augmentations/gaussian_loc.png}
         \caption{Gaussian Local $\nu$}
     \end{subfigure}
    \caption{\textbf{Examples of different augmentation methods.} (b)-(e) are examples from other augmentation baselines (\S~\ref{sec:baselines}), and (f)-(h) are examples from our FlowAug (\S~\ref{sec:flowaug}). }
    \label{fig:augmentations}
\end{figure*}

% \begin{figure*}[t]
%     \begin{subfigure}[t]{0.1\textwidth}
%          \begin{subfigure}[b]{\linewidth}
%              \centering \includegraphics[scale=1.5]{figures/augmentations/natural.png}
%          \end{subfigure}
%          \begin{subfigure}[b]{1\linewidth}
%              \centering \includegraphics[scale=1.5]{figures/augmentations/mixup.png}
%          \end{subfigure}
%          \caption{Original}
%     \end{subfigure}
%     \hfil
%     \begin{subfigure}[t]{0.1\textwidth}
%          \begin{subfigure}[b]{1\linewidth}
%              \centering \includegraphics[scale=1.5]{figures/augmentations/cutout.png}
%          \end{subfigure}
%          \begin{subfigure}[b]{1\linewidth}
%              \centering \includegraphics[scale=1.5]{figures/augmentations/cutmix.png}
%          \end{subfigure}
%          \caption{Mixup}
%     \end{subfigure}
%     \hfil
%     \begin{subfigure}[t]{0.1\textwidth}
%          \begin{subfigure}[b]{1\linewidth}
%              \centering \includegraphics[scale=1.5]{figures/baby_0049.png}
%          \end{subfigure}
%          \begin{subfigure}[b]{1\linewidth}
%              \centering \includegraphics[scale=1.5]{figures/flat_fish0045.png}
%          \end{subfigure}
%          \caption{Cutout}
%     \end{subfigure}
%     \hfil
%     \begin{subfigure}[t]{0.1\textwidth}
%          \begin{subfigure}[b]{1\linewidth}
%              \centering \includegraphics[scale=1.5]{figures/baby_0049.png}
%          \end{subfigure}
%          \begin{subfigure}[b]{1\linewidth}
%              \centering \includegraphics[scale=1.5]{figures/flat_fish0045.png}
%          \end{subfigure}
%          \caption{Cutmix}
%     \end{subfigure}
%     \hfil
%     \begin{subfigure}[t]{0.1\textwidth}
%          \begin{subfigure}[b]{1\linewidth}
%              \centering \includegraphics[scale=1.5]{figures/baby_0049.png}
%          \end{subfigure}
%          \begin{subfigure}[b]{1\linewidth}
%              \centering \includegraphics[scale=1.5]{figures/flat_fish0045.png}
%          \end{subfigure}
%          \caption{AutoAug}
%     \end{subfigure}
%     \hfil
%     \begin{subfigure}[t]{0.1\textwidth}
%          \begin{subfigure}[b]{1\linewidth}
%              \centering \includegraphics[scale=1.5]{figures/baby_0049.png}
%          \end{subfigure}
%          \begin{subfigure}[b]{1\linewidth}
%              \centering \includegraphics[scale=1.5]{figures/flat_fish0045.png}
%          \end{subfigure}
%          \caption{Ours (Globalmix)}
%     \end{subfigure}
%     \hfil
%     \begin{subfigure}[t]{0.1\textwidth}
%          \begin{subfigure}[b]{1\linewidth}
%              \centering \includegraphics[scale=1.5]{figures/baby_0049.png}
%          \end{subfigure}
%          \begin{subfigure}[b]{1\linewidth}
%              \centering \includegraphics[scale=1.5]{figures/flat_fish0045.png}
%          \end{subfigure}
%          \caption{ours gaussian}
%     \end{subfigure}
%     \hfil
%     \begin{subfigure}[t]{0.1\textwidth}
%          \begin{subfigure}[b]{1\linewidth}
%              \centering \includegraphics[scale=1.5]{figures/baby_0049.png}
%          \end{subfigure}
%          \begin{subfigure}[b]{1\linewidth}
%              \centering \includegraphics[scale=1.5]{figures/flat_fish0045.png}
%          \end{subfigure}
%          \caption{local mix?}
%     \end{subfigure}
    
%     \caption{\textbf{Differences between augmentation methods.} }
% \end{figure*}

==> cifar10_casestudy_fig.tex <==
% \begin{wrapfigure}{r}{1\textwidth}
\begin{figure*}
  \centering
     \includegraphics[width=1\textwidth]{figures/cifar10_bestworst_standard_autoaug_flowaug.png}
        \caption{\textbf{Class average performances (dark) and their worst subgroup performances (light).} Although standard CNN model can reach human-level accuracy (\textit{red line}), we find that the subgroup performances can be surprisingly low. Even after data augmentation, the same phenomenon remains (\textit{middle}). Our FlowAug can mitigate such phenomenon \textit{(right)}.} 
    \label{fig:case_study}
\end{figure*}
% \end{wrapfigure}\hfil

==> graphical.tex <==
\begin{figure*}[t]
     \centering
     \includegraphics[width=0.5\textwidth]{figures/graphical.png}
        \caption{\textbf{Graphical model depicting our disentanglement assumptions.}}
        \label{fig:graphical}
\end{figure*}

==> table.tex <==

\begin{table*}
 \caption{\textbf{Test accuracies, \emph{MacroStd} and Weighted Std.} $\Delta$ is the performance gain from ``Standard'' (baseline). Our approach consistently outperforms the baseline. Note that we only highlight the numbers better than all the other augmentation methods.}
  \begin{adjustbox}{max width=\textwidth}
   \begin{tabular}{lccc|cccc}
    \toprule
     & \multicolumn{3}{c}{Accuracy} & \multicolumn{2}{c}{MacroStd} & \multicolumn{2}{c}{Weighted Std}\\
     & CIFAR-10 ($\Delta$) & CIFAR10.1 ($\Delta$) & CIFAR-100 ($\Delta$) & CIFAR10 & CIFAR100 & CIFAR10 & CIFAR100\\
     \midrule
 Baseline &   95 & 88.25 & 78.52 & 2.24 & 12.24 & 3.45 & 16.44\\
 Mixup &   95.82(0.82) & 88.85 (0.60) & 76.99 (-1.53) & 2.17 &  11.94 & 3.02 & 16.75\\
 Cutout &   95.6 (0.60) & 89.7 (1.45)& 78 (-0.52) & 1.91 & 12.45 & 2.94 & 16.52\\
 Cutmix &   96.04 (1.04) & 90.2 (1.95)& 78.42 (-0.10) & 1.91 &  12.62 & 3.34 & 16.87\\
 AutoAug &   95.47 (0.47) & 89.8 (1.55) & 78.12(-0.40) & 2.11 &  11.74 & 3.54 & 16.3\\
 \midrule
 Ours (Trunc Gaussian on $\nu$) &  95.45 (0.45) &   89.25 (1.00) & 78.41 (-0.11) & 1.94 & 12.68 & 2.81 & 16.7 \\
 Ours (Mix $\nu$) &   93.43 (-1.57) & 85.5 (-2.75) & 71.42 (-7.1) & 2.5 & 13.27 & 4.21 & 18.46\\
 Ours (Mix $z$)   & 95.59 (0.59) & 89.3 (1.05)  &  78.07 (-0.45) & 1.99 &  \textbf{11.73} & \textbf{2.92} & \textbf{15.96}\\
  + Std         & 95.73 (0.73) & \textbf{90.2} (1.95) & 78.06 (-0.46) & \textbf{1.81} &  12.49 & \textbf{2.76} & 16.76\\
 Ours (Uniform on $z$) & \textbf{96.11} (1.11)&  \textbf{90.45} (2.20) &  \textbf{79.24} (0.72) & \textbf{1.83} &  12.17 & 2.98 & 16.57\\
 Ours (Trunc Gaussian on $z$)    & \textbf{96.23} (1.23) &    \textbf{90.25} (2.00) & \textbf{79.04} (0.52) & \textbf{1.91} &  12  & \textbf{2.82} & \textbf{16.23}\\
  + Std     & \textbf{96.04} (1.04)&   89.8 (1.55)  & \textbf{79.62} (1.10) & \textbf{1.65} & \textbf{11.55} & 3.08 & \textbf{16.02}\\
 + Std + Mix $z$  & \textbf{96.29} (1.29) & \textbf{91.2} (2.95)& \textbf{79.31} (0.79) & \textbf{1.66} & 11.78 & \textbf{2.71} & \textbf{15.92}\\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \label{tab:acc}
\end{table*}



==> table_BestLast_stdGrp.tex <==

% \begin{table*}
%   \caption{\textbf{Test results in \% (best/last epoch).} $\Delta$ is the performance gain from \emph{Standard} . Our approach consistently outperforms the baseline and we only highlight the numbers better than other augmentation methods. Note that we apply the models trained from CIFAR-10 to obtain CIFAR10.1 results without fine-tuning. }
%   \begin{adjustbox}{max width=\textwidth}
%   \begin{tabular}{lcccccc}
%     \toprule
%      & CIFAR-10 & $\Delta$ & CIFAR10.1 & $\Delta$ & CIFAR-100 &  $\Delta$\\
%      \midrule
%  Standard & 95.16 / 95   & - & 88.70 / 88.25 &   -   &  78.52 / 78.52 &  - \\
%  Mixup & 95.96 / 95.82   & 0.80/0.82 & 89.75 / 88.85 & 1.05/0.60 & 77.91 / 76.99 & -0.61/-1.53\\
%  Cutout & 95.94 / 95.6   & 0.78/0.60 & 90.4 / 89.7 & 1.70/1.45& 78.21 / 78 & -0.31/-0.52\\
%  Cutmix & 96.17 / 96.04  & 1.01/1.04 & 90.05 / 90.2 & 1.35/1.95& 78.87 / 78.42 & 0.35/-0.10\\
%  AutoAug & 95.82 / 95.47 & 0.66/0.47 & 89.85 / 89.8 & 1.15/1.55 & 78.57 / 78.12& 0.05/-0.40\\
%  \midrule
%  Ours (Mix $z$)                  & 95.98 / 95.59 & 0.82/0.59 &  90.35 / 89.3 & 1.65/1.05&  78.58 / 78.07 & 0.06/-0.45 \\
%   + Std                          & 96.15 / 95.73 & 0.99/0.73 &  90.25 / \textbf{90.2} & 1.55/1.95&  78.66 / 78.06&  0.14/-0.46\\
%  Ours (Uniform on $z$)           & 96.12 / \textbf{96.11} & 0.96/1.11&  90.35 / \textbf{90.45} & 1.65/2.20&  \textbf{79.45} / \textbf{79.24}&  0.93/0.72\\
%  + Std           &  \textbf{96.28} / \textbf{96.14}  & 1.12/1.14 &  \textbf{90.95} / \textbf{91.15} & 2.25/2.9 & \textbf{79.68} / \textbf{79.67} &  1.16/1.15 \\
%  + Std + Mix $z$           & \textbf{96.44} / \textbf{96.31} & 1.28/1.31 &  \textbf{91.05} / \textbf{91}  & 2.35/2.75 &  \textbf{79.68} / \textbf{79.51} &  1.16/0.99 \\
%  Ours (Trunc Gaussian on $z$)    & \textbf{96.23} / \textbf{96.23} & 1.07/1.23 &  90.15 / \textbf{90.25} & 1.45/2.00&  \textbf{79.3} / \textbf{79.04} &  0.78/0.52\\
%   + Std                          & \textbf{96.22} / \textbf{96.04} & 1.06/1.04&  \textbf{90.55} / 89.8 & 1.85/1.55&  \textbf{79.62} / \textbf{79.62}&  1.10/1.10\\
%  + Std + Mix $z$                 & \textbf{96.53} / \textbf{96.29}& 1.37/1.29 &  \textbf{90.75} / \textbf{91.2} & 2.05/2.95&  \textbf{79.99} / \textbf{79.54} &  1.18/0.79\\
%  \midrule
%  Ours (Trunc Gaussian on $\nu$) & 95.7 / 95.45 & 0.54/0.45 &  88.7 / 89.25 & 0.00/1.00&  78.5 / 78.41&  -0.02/-0.11\\
%  Ours (Mix $\nu$) & 94.22 / 93.43 & -0.93/-1.57 & 87.55/85.5 & -0.85/-2.75 & 74.05 / 71.42 & -4.47/-7.1 \\
%     \bottomrule
%   \end{tabular}
%   \end{adjustbox}
  
%   \label{tab:acc}
% \end{table*}


\begin{table}
  
  \begin{adjustbox}{max width=\linewidth}
  \begin{tabular}{lccc}
    \toprule
     & CIFAR-10 & CIFAR10.1 & CIFAR-100 \\
     & best / last & best / last & best / last \\
     \midrule
 Standard & 95.16 / 95.00   & 88.70 / 88.25 &  78.52 / 78.52 \\
 Mixup & 95.96 / 95.82   & 89.75 / 88.85 & 77.91 / 76.99 \\
 Cutout & 95.94 / 95.60   & 90.40 / 89.70 & 78.21 / 78.00 \\
 Cutmix & 96.17 / 96.04  & 90.05 / 90.20 & 78.87 / 78.42 \\
 AutoAug & 95.82 / 95.47 & 89.85 / 89.80 & 78.57 / 78.12\\
 \midrule
 Ours (Mix $z$)                  & 95.98 / 95.59 & 90.35 / 89.30 & 78.58 / 78.07 \\
  + Std                          & 96.15 / 95.73 & 90.25 / 90.20 &  78.66 / 78.06\\
 Ours (Uniform on $z$)           & 96.12 / 96.11 & 90.35 / 90.45 &  79.45 / 79.24\\
 + Std           &  96.28 / 96.14 &  90.95 / 91.15 & 79.68 / \textbf{79.67} \\
 + Std + Mix $z$           & 96.44 / \textbf{96.31} & \textbf{91.05} / 91.00 &  79.68 / 79.51 \\
 Ours (Trunc Gaussian on $z$)    & 96.23 / 96.23 &  90.15 / 90.25 & 79.30 / 79.04 \\
  + Std                          & 96.22 / 96.04 &  90.55 / 89.80 &  79.62 / 79.62\\
 + Std + Mix $z$                 & \textbf{96.53} / 96.29&  90.75 / \textbf{91.20} & \textbf{79.99} / 79.54\\
 \midrule
 Ours (Trunc Gaussian on $\nu$) & 95.70 / 95.45 &  88.70 / 89.25 &  78.50 / 78.41\\
 Ours (Mix $\nu$) & 94.22 / 93.43 & 87.55 / 85.50 & 74.05 / 71.42 \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \caption{\textbf{Test results in \% (best/last epoch).} $\Delta$ is the performance gain from \emph{Standard} . Our approach consistently outperforms the baseline and we only highlight the numbers better than other augmentation methods. Note that we apply the models trained from CIFAR-10 to obtain CIFAR10.1 results without fine-tuning. }
  \label{tab:acc}
\end{table}

\begin{table}
% \begin{wraptable}{1\linewidth}
 
 \centering
  \begin{adjustbox}{max width=1\linewidth}
  \begin{tabular}{lcccc}
    \toprule
       &  \multicolumn{2}{c}{MacroStd} &  \multicolumn{2}{c}{Weighted Std}\\
       & CIFAR10 & CIFAR100 & CIFAR10 & CIFAR100 \\
     \midrule
    Standard & 2.24 & 12.24 & 3.45 &16.44\\
    Mixup    & 2.17 & 11.94 &3.02 &16.75\\
    Cutout &  1.91 & 12.45  &2.94 &16.52\\
    Cutmix &  1.91 & 12.62  &3.34 &16.87\\
    AutoAug & 2.11 & 11.74  &3.54 &16.30\\
    \midrule
    Ours (Trunc Gaussian on $\nu$) & 1.94 & 12.68 & 2.81 &16.70\\
    Ours (Mix $\nu$) & 2.50 & 13.27 & 4.21& 18.46\\
    Ours (Mix $z$) & 1.99 & 11.73 & 2.92 &15.96\\
    + Std & 1.81 & 12.49  & 2.76 & 16.76\\
    Ours (Uniform on $z$)  & 1.83 & 12.17 & 2.98 & 16.57\\
    + Std           &  1.81  &   11.59 & 3.26 & 15.95 \\
    + Std + Mix $z$ & 1.86 &  \textbf{11.23} & 3.12 & 16.01 \\
    Ours (Trunc Gaussian on $z$) & 1.91 & 12.00 & 2.82 &16.23\\
    + Std & \textbf{1.65} & 11.55 & 3.08 & 16.02 \\
    + Std + Mix $z$ & 1.66 & 11.78 & \textbf{2.71} &\textbf{15.92}\\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \caption{\textbf{\emph{MacroStd} and Weighted Std.} Lower numbers represent lower subgroup performance variabilities and our algorithms can achieve the lowest.}
  \label{tab:var}
% \end{wraptable}
\end{table}

  
% \begin{table*}
%  \caption{\textbf{MacroStd.} $\Delta$ is the MacroStd deficit from ``Standard'' (baseline). Our approach consistently outperforms the baseline.}
%  \centering
%   \begin{adjustbox}{max width=\textwidth}
%   \begin{tabular}{lcccc|cccc}
%     \toprule
%       &  \multicolumn{4}{c}{Class} &  \multicolumn{4}{c}{Group}\\
%       & CIFAR10 & $\Delta$& CIFAR100 & $\Delta$ & CIFAR10 & CIFAR100& & \\
%      \midrule
%     Baseline & 2.24 & - & 12.24 & - & 3.83 & 19.16\\
%     Mixup    & 2.17 & 0.07 & 11.94 & 0.3 & 3.66& 19.29\\
%     Cutout &  1.91 & 0.33 & 12.45 & -0.21 & 2.81 & 19.6\\
%     Cutmix &  1.91 & 0.33 & 12.62 &  -0.38 & 3.95& 19.69\\
%     AutoAug & 2.11 & 0.13 & 11.74 & 0.5 & 3.68& 19.08\\
%     \midrule
%     Ours (Trunc Gaussian on $\nu$) & 1.94 & 0.3 & 12.68 & -0.44& 3.34& 18.84\\
%     Ours (Mix $\nu$) & & & & & & \\
%     Ours (Mix $z$) & 1.99 & 0.25 & \textbf{11.73} & 0.51& 3.19& 19.53 \\
%     + Std & \textbf{1.81} & 0.43 & 12.49 & -0.25 & 3.37 & 19.49\\
%     Ours (Uniform on $z$)  & \textbf{1.83} & 0.41 & 12.17 & 0.07 & 3.18 & 19.55\\
%     Ours (Trunc Gaussian on $z$) & \textbf{1.91} & 0.33 & 12 & 0.24& 3.26 & 19.04\\
%     + Std & \textbf{1.65} & 0.59 & \textbf{11.55} & 0.69 & 2.91 & 20.02\\
%     + Std + Mix $z$ & \textbf{1.66} & 0.68 & 11.78 & 0.46& 3.07 & 18.87\\
%     \bottomrule
%   \end{tabular}
%   \end{adjustbox}
  
%   \label{tab:var}
% \end{table*}
